The Ninth NTIRE 2024 Efficient Super-Resolution Challenge Report

This paper provides a comprehensive review of the NTIRE 2024 challenge, focusing on efficient single-image super-resolution (ESR) solutions and their outcomes. The task of this challenge is to super-resolve an input image with a magnification factor of x4 based on pairs of low and corresponding high-resolution images. The primary objective is to develop networks that optimize various aspects such as runtime, parameters, and FLOPs, while still maintaining a peak signal-to-noise ratio (PSNR) of approximately 26.90 dB on the DIV2K_LSDIR_valid dataset and 26.99 dB on the DIV2K_LSDIR_test dataset. In addition, this challenge has 4 tracks including the main track (overall performance), sub-track 1 (runtime), sub-track 2 (FLOPs), and sub-track 3 (parameters). In the main track, all three metrics (ie runtime, FLOPs, and parameter count) were considered. The ranking of the main track is calculated based on a weighted sum-up of the scores of all other sub-tracks. In sub-track 1, the practical runtime performance of the submissions was evaluated, and the corresponding score was used to determine the ranking. In sub-track 2, the number of FLOPs was considered. The score calculated based on the corresponding FLOPs was used to determine the ranking. In sub-track 3, the number of parameters was considered. The score calculated based on the corresponding parameters was used to determine the ranking. RLFN is set as the baseline for efficiency measurement. The challenge had 262 registered participants, and 34 teams made valid submissions. They gauge the state-of-the-art in efficient single-image super-resolution. To facilitate the reproducibility of the challenge and enable other researchers to build upon these findings, the code and the pre-trained model of validated solutions are made publicly available at https://github.com/Amazingren/NTIRE2024_ESR/.

==> affiliation.tex <==
\subsection*{Your team name}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:your_email@xxx.xxx}{your_email@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> sec_main/helper.tex <==
Bin Ren and
Yawei Li and
Nancy Mehta and
Radu Timofte and
Hongyuan Yu and
Cheng Wan and
Yuxin Hong and
Bingnan Han and
Zhuoyuan Wu and
Yajun Zou and
Yuqing Liu and
Jizhe Li and
Keji He and
Chao Fan and
Heng Zhang and
Xiaolin Zhang and
Xuanwu Yin and
Kunlong Zuo and
Bohao Liao and
Peizhe Xia and
Long Peng and
Zhibo Du and
Xin Di and
Wangkai Li and
Yang Wang and
Wei Zhai and
Renjing Pei and
Jiaming Guo and
Songcen Xu and
Yang Cao and
Zhengjun Zha and
Yan Wang and
Yi Liu and
Qing Wang and
Gang Zhang and
Liou Zhang and
Shijie Zhao and
Long Sun and
Jinshan Pan and
Jiangxin Dong and
Jinhui Tang and
Xin Liu and
Min Yan and
Qian Wang and
Menghan Zhou and 
Yiqiang Yan and
Yixuan Liu and
Wensong Chan and
Dehua Tang and
Dong Zhou and
Li Wang and
Lu Tian and
Barsoum Emad and
Bohan Jia and
Junbo Qiao and
Yunshuai Zhou and
Yun Zhang and
Wei Li and
Shaohui Lin and
Shenglong Zhou and
Binbin Chen and
Jincheng Liao and
Suiyi Zhao and
Zhao Zhang and
Bo Wang and
Yan Luo and
Yanyan Wei and
Feng Li and
Mingshen Wang and
Yawei Li and 
Jinhan Guan and
Dehua Hu and
Jiawei Yu and 
Qisheng Xu and
Tao Sun and
Long Lan and
Kele Xu and
Xin Lin and
Jingtong Yue and
Lehan Yang and
Shiyi Du and
Lu Qi and
Chao Ren and
Zeyu Han and 
Yuhan Wang and 
Chaolin Chen and 
Haobo Li and
Mingjun Zheng and
Zhongbao Yang and
Lianhong Song and
Xingzhuo Yan and
Minghan Fu and
Jingyi Zhang and 
Baiang Li and
Qi Zhu and 
Xiaogang Xu and
Dan Guo and
Chunle Guo and 
Jiadi Chen and
Huanhuan Long and 
Chunjiang Duanmu and
Xiaoyan Lei and
Jie Liu and
Weilin Jia and
Weifeng Cao and
Wenlong Zhang and
Yanyu Mao and
Ruilong Guo and
Nihao Zhang and 
Qian Wang and 
Manoj Pandey and 
Maksym Chernozhukov and 
Giang Le and 
Shuli Cheng and
Hongyuan Wang and
Ziyan Wei and
Qingting Tang and
Liejun Wang and
Yongming Li and
Yanhui Guo and 
Hao Xu and
Akram Khatami-Rizi and
Ahmad Mahmoudi-Aznaveh and
Chih-Chung Hsu and
Chia-Ming Lee and
Yi-Shiuan Chou and
Amogh Joshi and 
Nikhil Akalwadi and 
Sampada Malagi and 
Palani Yashaswini and 
Chaitra Desai and
Ramesh Ashok Tabib and 
Ujwala Patil and 
Uma Mudenagudi

==> team11_FireWork/affiliation.tex <==
\subsection*{FireWork}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> team11_FireWork/main.tex <==
\subsection{FireWork}

==> team15_Minimalist/affiliation_old.tex <==
\subsection*{Minimalist}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> team15_Minimalist/main_old.tex <==
\subsection{Minimalist}

==> team22_VIP/affiliation.tex <==
\subsection*{VIP}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\

==> team22_VIP/main.tex <==
\subsection{VIP}

==> team28_DASE-IDEALab/affiliation.tex <==
% \subsection*{DASE-IDEALab}
% \noindent\textit{\textbf{Title: }} Multi-Scale Attention Network\\
% \noindent\textit{\textbf{Members: }} \\
% Zhijian Wu$^1$ (\href{zjwu_97@stu.ecnu.edu.cn}{zjwu\_97@stu.ecnu.edu.cn}),\\
% Jingchao Wang$^1$, \\
% Dingjiang Huang$^1$, \\
% \noindent\textit{\textbf{Affiliations: }} \\ 
% $^1$ School of Data Science and Engineering, East China Normal University\\




==> team28_DASE-IDEALab/main.tex <==
% \subsection{DASE-IDEALab}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{team28_DASE-IDEALab/network.pdf}
%     \caption{\textit{Team Dase-IDEALab:} The overall architecture of multi-scale attention network (MSN).}
%     \label{fig:team_idea}
% \end{figure}

% \noindent
% \textbf{Network Architecture.}
% The DASE-LEDALab team proposes the Multi-scale Attention Network (MSN) for efficient image super-resolution. The overall architecture is shown in Fig. \ref{fig:team_idea}, which is based on MDRN \cite{mao2023multi}, the champion method of the model complexity track of NTIRE2023. The difference is that MSN uses SSConv as the basic building block, and it uses strip depth-wise convolution to replace vanilla depth-wise convolution for further parameter reduction. In addition, we equip MDSA with layer normalization, which not only stabilizes the training but also improves the performance with barely parameters and computational effort. Finally, we remove the popular \emph{Concat} operation in favor of using \emph{Add} operation for feature fusion, which helps further reduce the parameter and computational overhead of the model.

% \noindent
% \textbf{Training strategy.} The model is first trained from scratch with $384 \times 384$ patches randomly cropped from HR images from DIV2K and the first 10k images of LSDIR datasets. The batch size is set to 64. 
% The model is trained using Adam optimizer with L1 loss. The initial learning rate is set to $2 \times 10^{-3}$. The total number of iterations is 300k. Then, the L2 loss is used for fine-tuning with $640 \times 640$ HR patches and a learning rate of $5 \times 10^{-4} $ for 400k iterations.

==> team39_SPAN-T/affiliation.tex <==
\subsection*{SPAN-T}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> team39_SPAN-T/main.tex <==
\subsection{SPAN-T}

==> team45_hajnal/affiliation.tex <==
\subsection*{hajnal}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> team45_hajnal/main.tex <==
\subsection{hajnal}
